Online probabilistic label trees

We introduce online probabilistic label trees (OPLTs), an algorithm that trains a label tree classifier in a fully online manner without any prior knowledge about the number of training instances, their features and labels. OPLTs are characterized by low time and space complexity as well as strong theoretical guarantees. They can be used for online multi-label and multi-class classification, including the very challenging scenarios of one- or few-shot learning. We demonstrate the attractiveness of OPLTs in a wide empirical study on several instances of the tasks mentioned above.

==> pics/plt_model.tex <==
\begin{tikzpicture}[scale = 1,every node/.style={scale=1},
		regnode/.style={circle,draw,minimum width=1.5ex,inner sep=0pt},
		leaf/.style={circle,fill=black,draw,minimum width=1.5ex,inner sep=0pt},
		pleaf/.style={rectangle,rounded corners=1ex,draw,font=\scriptsize,inner sep=3pt},
		pnode/.style={rectangle,rounded corners=1ex,draw,font=\scriptsize,inner sep=3pt},
		rootnode/.style={rectangle,rounded corners=1ex,draw,font=\scriptsize,inner sep=3pt},
		level/.style={sibling distance=12em/#1, level distance=5ex}
	]
	\node (z) [rootnode] {$(1)$}
	child {node (a) [pnode] {$\bz^1 = (1,0)$} 
		child {node [label=below:{\makebox[1cm][c]{$y_1$}}] (b) [pleaf] {$(1,0,0)$} edge from parent node[above left]{}}
		child {node [label=below:{\makebox[1cm][c]{$y_2$}}] (g) [pleaf] {$(1,0,1)$} edge from parent node[above right]{}}
		edge from parent node[above left]{}
	}
	child {node (j) [pnode] {$(1,1)$}
		child {node [label=below:{\makebox[1cm][c]{$y_3$}}] (k) [pleaf] {$(1,1,0)$} edge from parent node[above left]{}}
		child {node [label=below:{\makebox[1cm][c]{$y_4$}}] (l) [pleaf] {$(1,1,1)$}
			{
				child [grow=right] {node (s) {} edge from parent[draw=none]
					child [grow=up] {node (t) {} edge from parent[draw=none]
						child [grow=up] {node (u) {} edge from parent[draw=none]}
					}
				}
			}
			edge from parent node[above right]{}
		}
		edge from parent node[above right]{}
	};
	\end{tikzpicture}
